GelSight Svelte: A Human Finger-shaped Single-camera Tactile Robot Finger with Large Sensing Coverage and Proprioceptive Sensing

Camera-based tactile sensing is a low-cost, popular approach to obtain highly detailed contact geometry information. However, most existing camera-based tactile sensors are fingertip sensors, and longer fingers often require extraneous elements to obtain an extended sensing area similar to the full length of a human finger. Moreover, existing methods to estimate proprioceptive information such as total forces and torques applied on the finger from camera-based tactile sensors are not effective when the contact geometry is complex. We introduce GelSight Svelte, a curved, human finger-sized, single-camera tactile sensor that is capable of both tactile and proprioceptive sensing over a large area. GelSight Svelte uses curved mirrors to achieve the desired shape and sensing coverage. Proprioceptive information, such as the total bending and twisting torques applied on the finger, is reflected as deformations on the flexible backbone of GelSight Svelte, which are also captured by the camera. We train a convolutional neural network to estimate the bending and twisting torques from the captured images. We conduct gel deformation experiments at various locations of the finger to evaluate the tactile sensing capability and proprioceptive sensing accuracy. To demonstrate the capability and potential uses of GelSight Svelte, we conduct an object holding task with three different grasping modes that utilize different areas of the finger. More information is available on our website: https://gelsight-svelte.alanz.info

==> body/2_related_works.tex <==
\section{Related Works}

Camera-based tactile sensors have the advantage of producing the geometry of the contact surface with high spacial resolution while keeping the form factor small and the cost low. 
One popular example of camera-based tactile sensors is the GelSight sensor, which relies on carefully designed LED illumination and the photometric stereo algorithm to reconstruct the 3D shape of the contact surface \cite{yuan2017gelsight}.
However, due to physical constraints such as size of the camera, focal distance of the lens, and viewing angles, most camera-based tactile sensors have the limitation of being flat, small and they lack a wide-range proprioceptive sensing ability.

% flat
\textbf{Most existing camera-based tactile sensors are flat.} 
Popular camera-based tactile sensors, including GelSight \cite{yuan2017gelsight}, GelSight Wedge \cite{wang2021gelsight}, and GelSlim 3.0 \cite{taylor2022gelslim} are all flat sensors. 
% There are mainly two reasons for this design choice: (1) they were primarily designed to replace the fingertip in parallel jaw grippers, so having a similar geometry with the original flat fingertips is desirable, and (2) 
The main reason for this design choise is that illumination needs to be well controlled for photometric stereo to work well, and it is easier to achieve better illumination with planar geometries.
The use case for flat tactile sensors is limited.
Imagine the way humans flip a coin that is lying flat on a table: we use the tip of one finger to stop the coin, then we use another finger's finger pad and tip to flip it.
It is nearly impossible to do this task with flat robot fingers without re-grasps or external contacts.
% The lack of sensing on the front and the side of flat tactile sensors makes this task challenging.
% Flat sensors also have the disadvantage of not being able to produce sensing signals when handling concave objects with cavities that are smaller than the finger itself.
Therefore, shape design for tactile sensors is important.
Romero et al. introduced a round sensor design utilizing a clear resin shell to create a pipe for light, which hereby controls illumination directions \cite{romero2020soft}.
The authors also demonstrated that such a round sensor was able to perform object rolling tasks. % more easily than flat sensors.

% small
\textbf{Most existing camera-based tactile sensors are fingertip sensors.} 
Tactile sensors introduced in \cite{yuan2017gelsight, wang2021gelsight, taylor2022gelslim, romero2020soft} are all fingertip sensors.
However, consider a human hand, where fingertips only constitute a very small portion of the sensing areas of the whole hand. 
For grasping modes such as lateral pinch grasps and power grasps, it is important to have sensing along the entire finger.
Existing solutions to increase sensing coverage include using wide-angle cameras and using multiple cameras.
Wilson et al. designed a robot claw with two fingers, where each finger has two sections and each section houses a GelSight style flat tactile sensor \cite{wilson2020design}.
Liu et al. introduced an exoskeleton-covered soft finger design \cite{she2020exoskeleton}, where 2 wide-angle cameras are placed inside a large piece of soft gel which constitutes the body of the finger.
Both tactile fingers introduced in \cite{wilson2020design, she2020exoskeleton} have a higher sensing coverage than traditional fingertip tactile sensors.
However, they both require 2 cameras per finger, which adds bulkiness and introduces new challenges for signal processing and signal synchronization.
Moreover, both sensors still lack sensing ability on the sides.
% Sun et al. introduced a cone-shaped tactile finger that has one wide-angle camera on the base where the camera can capture the entire inner surface of the cone-shaped elastomer \cite{sun2022soft}.
% However, due to physical constraints, the LED and the camera are placed very close to each other, meaning the illumination angle and the imaging angle are almost the same at each spot.
% This makes it hard for photometric stereo to capture height gradients from the contact surface.

% proprioceptical
\textbf{Proprioceptive information is generally hard to obtain with most camera-based tactile sensors.}
In addition to contact geometry inference, normal and shear force estimation provides unique insight into the stability of the contact.
% It is straightforward to obtain normal force and shear force measurements from tactile fingers built with arrays of force torque sensors \cite{tomo2017covering}.
It is possible to estimate normal and shear force on camera-based tactile sensors by printing markers on the elastomer surface \cite{yuan2017gelsight, wang2021gelsight, wilson2020design}.
The marker movement produces a vector field of forces on the contact surface, from which the local normal and shear force can be estimated.
However, force estimation through marker movement is hard to do when the contact shape is complex, because the marker movement is highly dependent on the contact texture, and the markers are usually sparse.
The sensing range and the resolution can also be limited if the gel is thin, and re-calibration will be needed if the gel stiffness is changed.

Therefore, it is desirable to have a tactile finger design that is curved, human finger-sized, and able to produce tactile sensing as well as proprioceptive sensing over a large area.
We present GelSight Svelte, a low-cost solution to this design goal. 
% GelSight Svelte utilizes reflection and refraction inside the finger to achieve the shape design goal and the sensing coverage goal.

